Deterministic Digital Clustering of Wireless Ad Hoc Networks

We consider deterministic distributed communication in wireless ad hoc networks of identical weak devices under the SINR model without predefined infrastructure. Most algorithmic results in this model rely on various additional features or capabilities, e.g., randomization, access to geographic coordinates, power control, carrier sensing with various precision of measurements, and/or interference cancellation. We study a pure scenario, when no such properties are available. As a general tool, we develop a deterministic distributed clustering algorithm. Our solution relies on a new type of combinatorial structures (selectors), which might be of independent interest. Using the clustering, we develop a deterministic distributed local broadcast algorithm accomplishing this task in $O(\Delta \log^*N \log N)$ rounds, where $\Delta$ is the density of the network. To the best of our knowledge, this is the first solution in pure scenario which is only polylog$(n)$ away from the universal lower bound $\Omega(\Delta)$, valid also for scenarios with randomization and other features. Therefore, none of these features substantially helps in performing the local broadcast task. Using clustering, we also build a deterministic global broadcast algorithm that terminates within $O(D(\Delta + \log^* N) \log N)$ rounds, where $D$ is the diameter of the network. This result is complemented by a lower bound $\Omega(D \Delta^{1-1/\alpha})$, where $\alpha > 2$ is the path-loss parameter of the environment. This lower bound shows that randomization or knowledge of own location substantially help (by a factor polynomial in $\Delta$) in the global broadcast. Therefore, unlike in the case of local broadcast, some additional model features may help in global broadcast.

==> conclusions.tex <==
We have shown that it is possible to build efficiently a clustering of an ad hoc network without use of randomization in a very harsh model of wireless SINR networks. Using the clustering algorithm, we developed a very efficient local broadcast algorithm. On the other hand, by an appropriate lower bound, we  exhibited importance of randomization or availability of 
%\deleted{geometric} 
coordinates for complexity of the global broadcast problem.
%
The exact complexity of global broadcast remains open as well as the impact of other features, e.g., carrier sensing or power 
\ifshort
control.
\else
control in
the deterministic setting.
\fi

We developed a combinatorial structure called \emph{witnessed (cluster aware) strong selector} along with several communication primitives, 
\ifshort
which might be of independent interest.
\else
which allowed for improving the complexity of our algorithms, and might be of independent interest.
\fi
\comment{
in a very harsh 
In the paper we presented two solutions to broadcast and local broadcast with complexity, respectively $O(n\log^2 n), O(D(\Delta+\log^* n)\log n)$ and $O((\Delta+\log^* n)\log^2 n)$. We gave a lower bound $\Omega(D\Delta^{1-1/\alpha})$ for the broadcast problem which separates determinism from randomness in an ad hoc setting. The local broadcast algorithm is a first deterministic solution to the problem and achieves the complexity which is close to best known randomized solutions. Moreover, we developed a combinatorial structure called \emph{eliminating selector} along with several communication primitives, which allowed for improving the complexity of our algorithms, and are of independent interest. 
}
